Orbital evolution of potentially habitable planets of tidally interacting binary stars

We simulate the coupled stellar and tidal evolution of short-period binary stars (orbital period $P_{orb} \lsim$8 days) to investigate the orbital oscillations, instellation cycles, and orbital stability of circumbinary planets (CBPs). We consider two tidal models and show that both predict an outward-then-inward evolution of the binary's semi-major axis $a_{bin}$ and eccentricity $e_{bin}$. This orbital evolution drives a similar evolution of the minimum CBP semi-major axis for orbital stability. By expanding on previous models to include the evolution of the mass concentration, we show that the maximum in the CBP orbital stability limit tends to occur 100 Myr after the planets form, a factor of 100 longer than previous investigations. This result provides further support for the hypothesis that the early stellar-tidal evolution of binary stars has removed CBPs from short-period binaries. We then apply the models to Kepler-47 b, a CBP orbiting close to its host stars' stability limit, to show that if the binary's initial $e_{bin} \gsim$0.24, the planet would have been orbiting within the instability zone in the past and probably wouldn't have survived. For stable, hypothetical cases in which the stability limit does not reach a planet's orbit, we find that the amplitudes of $a_{bin}$ and $e_{bin}$ oscillations can damp by up to 10\% and 50\%, respectively. Finally, we consider equal-mass stars with $P_{orb} =$ 7.5 days and compare the HZ to the stability limit. We find that for stellar masses $\lsim0.12M_{\odot}$, the HZ is completely unstable, even if the binary orbit is circular. For $e_{bin} \lsim$0.5, that limit increases to $0.17M_{\odot}$, and the HZ is partially destabilized for stellar masses up to $0.45M_{\odot}$. These results may help guide searches for potentially habitable CBPs, as well as characterize their evolution and likelihood to support life after they are found.

==> cuttingroom.tex <==


\begin{table}
\caption{Initial conditions for all simulations with exception to Figure \ref{steep}, which used the initial conditions from Table 1 of \citet{Fleming18}. Not all simulations contain a CBP, thus the CBP information is ignored for simulations without CBPs.}              % title of Table
\label{general_conditions}      % is used to refer this table in the text
\centering                                      % used for centering table
\begin{tabular}{c c}          % centered columns (2 columns)
\hline\hline                        % inserts double horizontal lines
Parametern & Value \\    % table heading
\hline                                   % inserts single horizontal line
    $r_g$ & 0.27 \\      % inserting body of the table
    Initial Age [Myr] & 1.0 \\
    Initial Stellar $P_{rot}$ [days] & 4.0 \\
    CBP mass [$M_{\oplus}$] & 2.98 \\
    Stellar Tidal $\tau$ [seconds] & 0.1 \\
    Stellar Love Number & 0.5 \\
\hline                                             %inserts single line
\end{tabular}
\end{table}

For all of our simulations there are some initial conditions that remain untouched. A general overview of initial conditions for all simulations is shown on Table \ref{general_conditions} with exception to Figure \ref{steep}, in which the initial conditions may be refered to the fiducial values in Table 1 of \citet{Fleming18}.
\begin{itemize}
    \item In general the primary star's mass in our simulations always remains below 1.1 \Msun, so we assume an initial $r_g$ of 0.27, since sun-like stars have this value, however higher values may be considered. \citet{Baraffe15} shows that low-mass stars may be as high as 0.45.
    \item The evolution of $r_g$ remains dynamic. The inertia of stars varies in the beginning of their evolution and is shown by comparison when the STEEP model from \citet{Fleming18} is turned on compared to when $r_g$ remains static as shown in Figure \ref{steep}. \acrit~ highly depends on the evolution of $r_g$.
    \item The initial age of the binary stars is set to 1.0 Myr since current dynamic models in are not yet certain of how stars evolve. Since the initial age is set to 1.0 Myr, all initial conditions are assumed to start at 1.0 Myr.
    \item Initial rotation periods vary from star to star, however a certain range of initial values is reasonable. In general we chose the initial rotation period $P_{rot}$ to be 4.0 days.
    \item CBP mass and radius can be ignored as long as the CBP's mass is much smaller than both of the binary stars. There is no special context to the value of 2.98 $M_\oplus$ and 2.98 $R_\oplus$, since one can choose a range values that can be much smaller than both of the stars.
    \item Tidal $\tau$ tends to range between 0.1 and 1 second. As tidal $\tau$ increases, the tidal lock time decreases, then causes \acrit~ to decrease at earlier times. \help{A source has claimed that a tidal $\tau$ of 0.1 seconds is much more reasonable than 1 second for stars.}
    \item The Love number is unitless quantity that defines the rigidity of a celestial object, where a Love number of 0 would define a malleable liquid of a celestial object and a Love number of 1 would define a stiff solid celestial object. Normally we accept that a Love number of a star contains a value of 0.5, since stars are normally assumed to be spherically gases, however become more rigid as the density increases towards the star's center.
\end{itemize}

In addition, the initial binary orbital period remain at a similar value between 7.0 to 7.5 days. the initial orbital period was chosen to be roughly 7.0 days since binary stars tend to return to their initial orbital period after the magnetic breaking process finishes decaying the binary orbit \help{I need a source from this last claim.} Our investigation revolves around the limit that no CBPs have been discovered orbiting tight-orbiting binary stars of less than 7.5 days, which is why our initial binary orbital period was chosen to be 7.5 days.


\subsection{Tidal Time Lag VS. Binary Eccentricity}

Tidal taus ($\tau$) of tidally interacting stars were examined in order to see if their values had any significant effects on the eccentricity of CBPs. The results were not so dramatic; the envelope enclosing the oscillation of the CBP's free eccentricity were mostly flat without signs of damping, however the scenario of $\tau = 0.01 s$ and $e_0 = 0.4$ involved an increase in amplitude during the beginning of its evolution followed by some damping effect, where the damping stopped at roughly the same amplitude as the amplitude of the simulation with conditions of $\tau = 0.1$ and $e_0 = 0.4$. 

There is something worthy of how $\tau$s affect the evolution of \acrit~ and thus affecting the dynamics of CBPs when consider the CTL model. $\tau$ affects the time in which \acrit~ may decrease.  Referring to Figures \ref{k47b} and \ref{habtiablecbp}, the envelopes of \acbp and \ecbp are affected by the difference between the average of \acbp and \acrit. As the difference decreases, the amplitudes of \acbp and \ecbp increase, therefore if \acrit~ stays more or less constant throughout the time evolution, the amplitudes of \acbp and \ecbp will also stay constant. Higher values in $\tau$ lead to a stronger tidal interactions between the stars, thus leading to a faster tidal lock time. By no means does $\tau$ affect $a_{star, max}$ nor $e_{star, max}$; $\tau$ affects the time it takes for the two stars to tidally lock. After tidal locking, the binaries begin to circularize due to magnetic breaking. Since \cite{Holman99} show that \acrit~ depends on $e_{star}$, then \acrit~ decreases during the process as well. A much stronger dependence than $\tau$ is the stellar orbital period. Tighter orbits call for a stronger gravitational interaction in tidal torques. For $\tau$ between 0.1 and 0.9 stellar initial orbital periods ($P_{0}$) of 5 days drop dramatically before the first billion of the binary stars' existence. At $P_{0} = $ 14 days the drop in binary eccentricity begins between 0.1 and 1 Gyr. At $P_{0} = $ 20 days Binary eccentricities only begin their slow decline in eccentricity well after a billion years and barely make a difference even after 10 billion years. While $\tau$ does make a difference as to how soon the binary stars tidally lock, stellar orbital periods participate in a bigger role as to when \acrit~ may drop. As $\tau$ decreases, the time it takes for the binary star to circularize increases. We chose a conservative value of $\tau = 0.1s$ for our simulations.


but prefer to maintain a dynamic radius of gyration (\rg) for all of our simulations. We show that the STEEP model from \citet{Fleming18} dramatically increases the binary orbital period and binary eccentricity, which consequently increases \acrit relative to a static \rg. Because \rg evolution increases \aratio, we find it reasonable to assume the rest of our simulations to have a dynamic evolution.

Section 3.3 (Kepler-47) introduces a real-life example of a tight-orbiting CBP. We model a potential long-term evolution scenario of K47's closest CBP, K47 b as \acrit evolves within close proximity to the CBP (Figure \ref{k47b}) while the CBP maintains dynamic stability throughout the entire evolution. We create initial conditions in which the simulation could evolve in the present-day values of K47 ($a_{K47B}$, $a_{K47b}$, \acrit, $e_{K47B}$, $e_{K47b}$). In addition we provide evidence that indicates the initial binary eccentricity of K47AB must be low ( $\lessapprox 0.25$) in order for K47b to exist. If K47b would hypothetically go unstable, then the CBP would go unstable within the first tens of millions of years of K47's evolution and decreasing to zero as the initial binary eccentricity increases. The tidal lock time of K47B remains constant while K47A initially remains low, spikes up to a few Gyrs, and decreases as the initial binary eccentricity increases.

Section 3.4 (Long-Term CBP Orbital Evolution) applies the evolution of \acrit~ into theoretical examples of binary HZs interacting with \acrit~ and that \acrit~ narrows binary HZs. HZ boundaries and \acrit~ vary throughout time and \amax~ can replace the inner boundary of HZs, thus narrowing the HZ, if not permanently removing the HZ throughout all time after \amax was reached. Present-day dynamically stable binary HZs may be present in once dynamically unstable environments, rendering vacancy of CBPs in binary HZs. We also show an example of a potentially habitable CBP in which the initial conditions were chosen so that the dynamics of the CBP were most variable throughout the evolution.

Section 3.5 (Stability of the Circumbinary HZ) \citet{Welsh2014} has shown that there have not been any presense of CBPs orbiting binaries with orbital periods of less than 7.5 days. In this section we show a different perspective of how \acrit limits dynamically unstable HZs. We demonstrate that \acrit highly depends on the binary eccentricity of the star. higher binary eccentricities increases the \acrit boundary and then could more likely interfere with HZs. Our HZs are limited to equal-mass binary stars since there has not been a confirmed model of nonidentical binaries.


the stars are identical, and it is worth noting that even though \cite{Baraffe15} proposes that low-mass stars begin with a high \rg~ value of 0.45, we maintain an initial value for \rg~ and remain with the fiducial value of 0.27 to preserve a conservative outcome for \aratio.\\

Consider conservation of angular momentum for a moment, where we have the sum of orbital angular momentum and rotational angular momentum. Using stellar tidal forces as the bridge that translates rotational angular momentum to orbital angular momentum, even if \rg~ is kept as constant, the stars would be able to translate more rotational angular momentum to the orbital angular momentum.

If \rg~ is dynamic, \aratio should increase significantly compared to when \rg~ is static. \rg~ should decrease over the evolution of a star. Figure \ref{steep} also shows how a dynamic \rg~ significantly raises \aratio compared to when \rg~ is static, therefore the evolution of \rg~ significantly contributes to the STEEP process in which CBPs orbiting in close proximity to \acrit face a higher likelihood of becoming ejected from their star systems.





 We show this relation on Figure \ref{steep}, where the binary eccentricity (\ebin) and semi-major axis (\abin) are values proportional to a star's orbital angular momentum. Since we show that \ebin and \abin increase in both cases where \rg~ is either static or dynamic, then \aratio must also increase as shown on the left panel. 

While the maximum value for \acrit results in a similar value for both the CTL and CPL model under a constant \rg~ value, the \aratio  value for the CTL model is higher than the CPL model. The same pattern shows when comparing the models with their maximum \ebin  and \abin. The qualitative results for the evolution may be the same when using either CTL or CPL models, however in both the dynamic and static simulations for \rg, the CTL reaches its maximum \acrit before the CPL reaches its maximum value, with the CTL roughly peaking at $10^7$ years and the CPL model peaking just after $10^8$ years. 

To date there have been no discoveries of CBPs orbiting around tight-orbiting binary stars with binary orbital periods of less than 7.45 days. Kepler-47 (K47) is a great example of CBPs orbiting incredibly close to the short period binary stars, since its closest orbiting CBP, Kepler-47 b (K47b) has an orbital period of 49.5 days \cite{Orosz12}, almost touches \acrit, and holds the record for orbiting the shortest orbiting binary stars with CBPs \cite{Winn15}. K47 is also the only know binary star system with multiple CBPs. It is not known whether the other discovered binary systems with CBPs contain more than one CBP, however CBP formation should be similar compared to the formation of planets orbiting single stars \cite{Vartanyan16}.

In this section, we assume that the gravitational influence of K47b is strictly dependant upon its host stars Kepler-47 A and B; we ignore the gravitational influence of the other CBPs in the system. Ignoring planetary migration is a reasonable assumption, since migration tends to occur during the first millions years of the binary stars' existence \cite{Pierens07}. The CBP's oscillation in eccentricity ($e_{cbp}$) and semi-major axis ($a_{cbp}$) depend much more on how close the CBP is to \acrit, however the dampening of K47b's oscillatory envelope does not depend much on the initial conditions of the binary stars, which is the binary eccentricity. The CBP's total eccentricity depends on the sum of the forced eccentricity and the free eccentricity ($e_{cbp, free}$), an eccentricity which is kept constant. The dampening of amplitudes in \acbp and \ecbp is less prominent when stars are more identical in mass. The initial conditions of the CBP such as $e_{cbp, free}$ and the distance between $a_{cbp}$ and \acrit~ play a bigger role in the CBP's own dampening. Our simulations have shown that CBPs with incredibly low initial $e_{cbp, free}$ contain dampening effects on $a_{cbp}$ and $e_{cbp, free}$. The CBP appears to dampen to its original initial conditions when $a_{crit}$ starts distancing itself from the CBP. From our CBP dynamic simulations, even with an initial $e_{cbp, free}$ as low as 0.05 will not dampen if their amplitudes are significantly low.

In relation to Kepler 47, dynamic evolution varies more throughout time when the difference between the primary and secondary star mass increases, because dampening effects tend to increase as the difference in primary and secondary mass increases. Kepler 47 is a planet with a primary stellar mass of $M_{1} = 1.043 M_{\odot}$ and a secondary stellar mass of $M_{2} = 0.362 M_{\odot}$ \cite{Orosz12}.

After experimenting with many initial conditions of CBPs and binary stars, we found that binary eccentricity makes the biggest impact in the dynamic evolution of binary stars with their tight-orbiting CBPs, due to the strong influence that binary eccentricity has on \acrit. The analysis that we explored in K47b by using the CTL model allowed us to show that if the initial binary eccentricity of system were ever higher than $0.236$ as shown on Figure \ref{K47_Eccentricities}, then K47b would not survive the long-term evolution, since $a_{crit}$'s time-evolution would have destabilized the CBP. We are also assuming that we're ignoring CBP migration.

Figure \ref{K47_Eccentricities} visualizes the evolution of \acrit~ for initial binary eccentricities between 0.10 and 0.49. Initial \ebin greatly effect the value of $a_{crit, max}$ in each simulation. Keep noted that the current value for \acrit~ $-$ \acbp is approximately -0.09 AU. As shown on Figure 9 in \cite{Fleming18}, the ratio \aratio should increase as the binary eccentricity increases.

The middle panel of Figure \ref{K47_Eccentricities} envisions that if \acrit~ does reach the semi-major axis of \acbp, K47b quickly becomes unstable during its existence, with a maximum survival age of 33.6 Myrs and the time of instability quickly approaches zero as binary eccentricity increases. For any time during K47's evolution using the initial conditions of Table \ref{K47table}, \acrit~ $=$ \acbp at the beginning of the evolution when the initial \ebin is more than 0.43, however the instability timescale is already incredibly close to zero when the initial \ebin is 0.31. The middle panel of Figure \ref{K47_Eccentricities} concludes that instability occurs rapidly in the first tens of millions of years of K47b's existence.

The bottom panel of Figure \ref{K47_Eccentricities} shows the lock times of both K47A and K47B. An initial \ebin higher than 0.20 shows that K47A drops in Lock Time from 3.93 Gyrs to zero. K47B's lock time almost remains constant relative to K47A's lock time, but K47B shows a similar trend where lock time is suddenly apparent at \ebin $=$ 0.12 at a lock time of 169 Myrs and slowly drops to 124 Myrs at \ebin $=$ 0.49. Higher eccentricities encourage a quicker lock time and is directly related to the differential equations of \cite{Hut81}.

If K47b ever experienced any inward migration, then it would have the opportunity to start migrating inwards when \ebin and \abin start dropping, making \acrit drop as well, which is when the stars tidally lock and start circularizing. When setting the initial \ebin to 0.5, $a_{crit, max} = 0.33$AU. Setting the initial stellar orbital period to a value higher than 11 days already limits the time range K47b would need in order to migrate inwards, with \ebin starting to drop when the K47 stars are billions of years old. Even setting a high tidal $\tau$ value of 0.9 would still take billions of years for K47 stars to start circularizing.

Our $\tau$ value stated on Table \ref{K47table} is a conservative value and considered low. looking at higher $\tau$ values with an initial orbital period like the K47 stars make \ebin drop throughout all time, circularizing at a little over a billion years of K47's existence. If we set an initial \ebin higher than 0.236, then higher $\tau$ values are preferred in order allow more time for K47b to migrate inward. If planetary migration is insignificant and non-existent for K47b, then by keeping the initial \ebin to be less than 0.236, one could effectively use the CPL model to simulate the time evolution of K47b since the CTL model confirms that at high initial \ebin values, K47b would always be rendered unstable at some point during the binary's dynamic evolution.

on Figure \ref{k47b}, $a_{obs} = a_{sim}$ at 2Gyrs while $e_{obs} = e_{sim}$ at 4Gyrs, however we can adjust the simulated values of $a_{sim}$ and $e_{sim}$ to match the observed values at the exact same simulation time by tweaking the tidal $\tau$ so that both observed values equal the simulated values at the same time. We found that tweaking these values was not worth the effort since we don't know the precise age of K47 and the qualitative outcome is still preserved when avoiding these tweaks.



 We do try to explore the concept of nonidentical binary stars and at least try to imagine of what it is like for a potential Earth-like CBP to exist within the borders of \acrit, which is represented by referring to Figure \ref{habtiablecbp}. 
 
 The evolution of \acrit~ for equal-mass binary stars evolve in a way such that \acrit~ rises during the pre-main sequence of low-mass binary stars and after tidal locking, \acrit decreases due to the binaries circularizing. We would like to demonstrate a potentially habitable CBP where the amplitudes of \acbp and \ecbp vary throughout its time evolution. What conditions do the CBP and the binary stars require in order for the dynamic amplitude variations to be the most emphasized?\\
A key to vary the amplitudes of a CBP is that the smaller the difference between the average of \acbp and \acrit~ become, the higher the CBP's amplitude in \acbp and \ecbp rises. Throughout the CBP evolution, the CBP oscillates around the its average \acrit (The average \acrit~ happened to be the initial \abin~ for our simulations), so in order to vary the dynamic amplitudes of the CBP over time, we need to vary \acrit~ over time. The dynamics of \acrit~ in Figure \ref{k47b} compared to Figure \ref{hzevolution} already give a hint as to how \acrit~ may vary throughout time. We have discovered that the difference between the masses of the primary and secondary star can cause the \acrit~ to vary throughout its evolution. Figure \ref{hzevolution} shows a roughly flat evolution after \acrit~ has reached its maximum value and only decreases after the stars tidally lock. The masses of the primary and secondary stars of Kepler-47 A and Kepler-47 B (K47A and K47B) are 1.043\Msun and 0.362\Msun \cite{Orosz12}. The time evolution of \acrit~ for K47 in Figure \ref{k47b} shows a roughly flat evolution in \acrit~ at 1 Myr, except \acrit~ keeps rising until it peaks at about $50 Myrs$ and then decreases, creating a rising bump compared to the \acrit~ evolution in Figure \ref{hzevolution}. We considered the differences in between the primary and secondary star masses in order to vary the evolution of \acrit~ for our hypothetically habitable CBP in Figure \ref{habtiablecbp}. Varied the masses of the primary and secondary stars while at the same time trying to place the CBP as close as possible to \amax inside its potential HZ. We do not have a model that shows our CBP is in the HZ of the system, for now we demonstrate the total instellation in Earth units that the CBP receives by the binaries as shown on the top panel of Figure \ref{habtiablecbp}. While we cannot directly confirm the CBP is in the HZ, the instellation oscillates between 0.5 and 0.6 Earth units at the beginning of the main sequence and appears to start converging to 0.575. Effective stellar fluxes between 0.4 and 0.8 certainly in the HZ for stars with effective temperatures between 2600$K$ and 7200$K$ are always in the HZ as shown in Figure 8 from \cite{Kopparapu13}, thus we can only compare the instellation to the effective stellar flux and roughly claim that the CBP is orbiting within the HZ.\\
A similar pattern emerges when comparing the evolution of \acrit~ to the evolution of \ecbp. The upper envelope of \ecbp follows a similar rise and decline that \acrit~ makes. The same phenomena happens as well when comparing \ebin and \acrit~ in Figure \ref{k47b}.\\ 
The evolution of \acrit~ for nonidentical-mass binaries compared to identical-mass binaries could be different due to the time it takes for both stars to tidally lock. Identical-mass binary stars with the same initial rotation period tidally lock at the same time, while nonidentical-mass binaries with the same initial conditions tidally lock at different times (refer back to the bottom panel of Figure \ref{K47_Eccentricities}), which can cause \ebin to keep rising.\\
A final discovery that we found was that low CBP free eccentricities (\efree) of less than 0.05 tend to vary in amplitude over the time evolution. The closer \efree gets to zero, the more flat the bottom of the \ecbp envelope becomes. The initial \efree for Figure \ref{habtiablecbp} has $e_{free} = 0.0$ and contains a flat bottom envelope when looking at the CBP's eccentricity and only begins to drop after the binaries tidally lock. As \acrit~ migrates farther away from the CBP, \ecbp converges to \efree. A similar story occurs for K47b's eccentricity. K47b was given an \efree of 0.04, during K47b's evolution, the bottom envelope of K47b's eccentricity was not flat compared to our potentially habitable CBP in Figure \ref{habtiablecbp}, which was due to the difference in \efree. K47b's eccentricity then appears to converge to its given \efree after \acrit~ decreases over time. 



Section 3.2 applied the dynamics of binary stars and tight-orbiting CBPs to a real-life example, Kepler-47. We would like to further explore theoretical examples of how dynamic instability limits prohibit the existence of CBPs within the HZs of binaries. We refer to the dynamic stability limits of CBPs (\acrit) from \cite{Holman99} superimpose \acrit~ on our assumed HZ limits. We defined multiple \acrit~ with varying binary eccentricities in order to show how higher binary eccentricities infiltrate deeper into the HZs of identical binaries. Figure \ref{hzcbp} illustrates that \acrit~ highly depends on the eccentricity of the two binary stars. Qualitatively, we can be certain that any CBP crossing the black line ($e_{star} = 0$) over to the left at any eccentricity would for certain become ejected by the binary stars, since zero binary eccentricity would indicate the lowest possible boundary for any closely interacting binary star system. The minimum \acrit~ (\amin) is when the binary stars have an eccentricity of zero.

Any scenario in Figure \ref{hzcbp} must have $\mu = 1/2$, since the plot refers to equal-mass binaries, but the masses of the stars affect this boundary because \acrit~ is proportional to the semi-major axis, which is only dependent on the sum of the two stellar masses ($M_{TOT}$) due to Kepler's third law keeping the binary orbital period constant, thus \acrit$\propto M_{TOT}^{1/3}$.

We obtain essential information from Figure \ref{hzcbp} such that stellar masses of less than 0.12\Msun have their HZs completely engulfed by \amin, which also means that any higher eccentricity would pose an even higher threat to CBPs that attempt to orbit within the HZs of 0.12\Msun binaries. Binaries with \amin contain partially dynamically unstable HZs from 0.12\Msun to about 0.28\Msun, therefore any identical binaries above 0.28\Msun would have completely dynamically stable HZs. Dynamic stability limits increase with binary eccentricity, the partially unstable HZ limits of 0.12\Msun to 0.28\Msun increase from 0.18\Msun to 0.47\Msun respectively when \ebin $= 0.5$. More details on stability limits infiltrating HZs are shown on Table \ref{limitshzcbp}. Identical tight-orbiting M-dwarf binaries would pose a difficult task in trying to contain a CBP in long-term dynamic stability.

We find that as the masses of the binary stars becomes less identical, the higher \amax becomes during the binary stars' evolution. For nonidentical mass binaries we are assuming both stars initially begin with the same rotational period. Both stars experience the same tidal torque before any of the stars tidally lock.

Figure \ref{hzcbp} illustrates that \acrit~ infiltrates the HZ of identical low-mass binaries; however, we are only observing dynamic stability limits for only a snapshot of time. It is important to know how \acrit~ and the HZ limits change over time, since stellar evolution will greatly affect the change in \acrit~ and the HZ limits. Once again, we will have some constraints as to how we can analyze the evolution of \acrit~ and the HZ. We must consider equal-mass binary stars in order to model the HZ. Referring to figure \ref{hzcbp} as a guide to simulating the evolution of \acrit~ with the HZ boundaries, binary stellar masses of 0.2\Msun and less have a major conflict with CBPs being able to orbit within the HZ and from 0.4\Msun and above, the HZ starts to become more dynamically stable for CBPs, even for binary eccentricities up to 0.5.

Since we considered $e_{star,0} = 0.3$ the CTL model would compliment the ability to support our defined initial eccentricity, in which $e_{star,0}$ was chosen due to population models shown on figure 15 from \cite{Raghaven10}, where the binary eccentricity distribution for binary orbits seems common for $0.2 \lessapprox e_{star,0} \lessapprox 0.6$. On the top panel of Figure \ref{hzevolution}, \acrit~ completely eliminates any sort of possibility of a CBP to orbit within the HZ for low stellar binary masses of 0.15 and \acrit~ completely eliminates any possibility for CBPs to exist within the HZ during the entire 10 Gyr evolution since \acrit~ remains roughly equal to \amax for the entire simulation. Even if \acrit did start to drop earlier, then it would have to significantly need to decrease its semi-major axis in order for the HZ to become dynamically stable, the stars would need to have higher tidal $\tau$ values, or the initial stellar rotation period would need to be increased. Low-mass tight-orbiting red dwarfs will never be able to sustain an Earth-like CBP, even considering that the error of up to $6\%$ for the \cite{Holman99} dynamic stability limit, the HZ is incredibly submerged under the \acrit.\\
The middle of panel of $M = 0.3M_{\odot}$ almost covers all of the HZ during the main sequence phase, but the dynamic stability limit begins to drop. An observer still wouldn't find a single CBP in this case, because during the binary star's early evolution ($<1 Gyr$), $a_{crit, max}$ peaked at a point where it covered the semi-major axis of the outer HZ limit during the main sequence. If planetary migration would allow a CBP to orbit closer to its host stars, the CBP's window of opportunity would seem small, especially since it appears that $a_{crit}$ would allow some slightly reasonable invitation to the HZ after $5 Gyrs$. While there may be a HZ that is dynamically stable for CBPs, their presence still appears vacant.

At $M = 0.45M_{\odot}$, the bottom panel of Figure \ref{hzevolution} allows for opportunities to arise for CBPs to maintain stable orbits within the HZ without $a_{crit, max}$ severely limiting the HZ. At this point, one could become more optimistic when searching for CBP's orbiting equal-mass binary stars of more than $0.45M_{\odot}$. 

One can hold \amax roughly constant by varying the initial stellar orbital and rotation periods. As the initial stellar orbital and rotation period of the binaries decrease at their own rate, \amax can remain constant, however \amax occurs at different times during the evolution. decreasing the initial stellar orbital and rotation period while \amax remains causes \amax to occur at earlier times, which causes \acrit~ to decrease earlier. The early decrease in \acrit~ concludes that one may observe vacant HZs due to the early intrusion of \amax. If the \amax occurred at roughly $1 Gyr$, then it's likely that \acrit~ would remain roughly fixed at \amax during the main-sequence, showing that potential HZs are actively intruded by by \acrit. 

We have used the STEEP model to show a dynamic radius of gyration (\rg) increases \amax much more than when \rg remains static. Qualitatively both the CTL and the constant phase-lag tidal equilibrium model (CPL) contain a higher \amax when our model has a dynamic \rg compared to a static evolution.

We superimposed the dynamic stability limit of CBPs orbiting tight-orbiting equal-mass binaries to their the binary's HZ to show how \acrit invades the HZ, rendering the HZs of binaries of less than 0.12\Msun to be completely dynamically unstable for CBPs and that increasing the binary eccentricity increases \acrit to further into HZs of higher stellar masses. We have also shown that dynamically stable HZs in the main sequence of low-mass tight-orbiting binaries may be still be deserted of CBPs due to \acrit's increased value during the PMS.\\

-- Our analysis for Kepler-47 b (K47b) was really comparison with what could currently do best with our coupled theoretical models. K47b was only simulated by ignoring the gravitational perturbations. In reality, the Kepler-47 binary star system contains three CBPs: Kepler-47 b, c, and d. The gravitational perturbations on K47b may be significant enough to cause a long-term effect in planet-to-planet migration within the system. Our goal for this investigation was analyze the effects of CBPs within close proximity to \acrit and assuming planetary migration occurred before CBPs settled in on their current orbital path. Future interests would be of course to study the dynamics of multiple CBPs gravitationally perturbing each other's orbits.  We found that for an intial \ebin of more than 0.236, K47b becomes dynamically unstable during the first tens of millions of years and even less as the intial \ebin increases. Given how K47b would quickly become unstable during its early life, it would be worth investigating several instability timescales for different scenarios. Is it a common that dynamic instability always occurs as early in the first tens of millions of years or may the instability timescale be extended to much higher quantities? 
